An adaptively inexact first-order method for bilevel optimization with application to hyperparameter learning

Various tasks in data science are modeled utilizing the variational regularization approach, where manually selecting regularization parameters presents a challenge. The difficulty gets exacerbated when employing regularizers involving a large number of hyperparameters. To overcome this challenge, bilevel learning can be employed to learn such parameters from data. However, neither exact function values nor exact gradients with respect to the hyperparameters are attainable, necessitating methods that only rely on inexact evaluation of such quantities. State-of-the-art inexact gradient-based methods a priori select a sequence of the required accuracies and cannot identify an appropriate step size since the Lipschitz constant of the hypergradient is unknown. In this work, we propose an algorithm with backtracking line search that only relies on inexact function evaluations and hypergradients and show convergence to a stationary point. Furthermore, the proposed algorithm determines the required accuracy dynamically rather than manually selected before running it. Our numerical experiments demonstrate the efficiency and feasibility of our approach for hyperparameter estimation on a range of relevant problems in imaging and data science such as total variation and field of experts denoising and multinomial logistic regression. Particularly, the results show that the algorithm is robust to its own hyperparameters such as the initial accuracies and step size.

==> siamart_220329/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{lipsum}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{graphicx}
\usepackage[numbers]{natbib}
\usepackage{doi}
\usepackage{graphicx}
\usepackage{array}
% \usepackage[dvipsnames]{xcolor}
% \usepackage{amsmath}
\usepackage{amssymb}
\usepackage{cases} % Include the cases package in your preamble
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{bbm}
\usepackage{float}
\usepackage{mathtools}
\usepackage{setspace}
%\usepackage{natbib}
\usepackage{natbib}
% \usepackage{amsmath}
\usepackage{newtxmath}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs = false}
\usepackage{cases} % Include the cases package in your preamble

\usepackage{doi}
% \usepackage{amsthm}
\usepackage{cases}
\usepackage{empheq}
% \usepackage{geometry}
\usepackage{caption}
\usepackage{algorithm}% http://ctan.org/pkg/algorithms
%\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage[noend]{algpseudocode}

\usepackage{subcaption}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamthm{assumption}{Assumption}


% Sets running headers as well as PDF title and authors
\headers{An adaptively inexact first-order method for bilevel optimization}{M. S. Salehi, S. Mukherjee, L. Roberts, M. J. Ehrhardt}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An adaptively inexact first-order method for bilevel optimization with application to hyperparameter learning \thanks{Submitted to the editors DATE. 
\funding{The work of Mohammad Sadegh Salehi was supported by a scholarship from the EPSRC Centre for Doctoral Training in Statistical Applied Mathematics at Bath (SAMBa), under the project EP/S022945/1. Matthias J. Ehrhardt acknowledges support from the EPSRC (EP/S026045/1, EP/T026693/1, EP/V026259/1). Lindon Roberts is supported by the Australian Research Council Discovery Early Career Award DE240100006.}}}

% Authors: full names plus addresses.
\author{Mohammad Sadegh Salehi\thanks{Department of Mathematical Sciences, University of Bath, Bath, BA2 7AY, UK (\email{mss226@bath.ac.uk}).}\and Subhadip Mukherjee\thanks{Department of Electronics \& Electrical Communication Engineering, Indian Institute of Technology (IIT), Kharagpur, India (\email{smukherjee@ece.iitkgp.ac.in}).} \and Lindon Roberts\thanks{School of Mathematics and Statistics, University of Sydney, Camperdown NSW 2006, Australia (\email{lindon.roberts@sydney.edu.au)}.} \and Matthias J. Ehrhardt \thanks{Department of Mathematical Sciences, University of Bath, Bath, BA2 7AY, UK (\email{m.ehrhardt@bath.ac.uk})}.}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

